Cosmic-ray propagation and production of secondary particles in the Galaxy

Cosmic rays are nowadays a crucial tool to study the astrophysics of extreme objects in the Universe, the cosmic environmental plasma (both Galactic and extra-galactic), the physics of nuclear interactions or the properties of elementary particles at very high energies and even cosmological problems such as the dark matter puzzle. In this thesis, the phenomenology on the transport of Galactic cosmic rays is studied in light of the most recent experimental data in the field and new analyses are presented in order to obtain better constraints. Throughout the thesis, secondary particles produced from collisions of cosmic rays with the interstellar gas, such as secondary cosmic ray nuclei (B, Be and Li), antiprotons and gamma rays, are treated in order to adjust and test our models and probe different scenarios, such as possible signatures of dark matter decay or annihilation. A preliminary version of the upcoming DRAGON2 code has been used to perform the propagation computations. With the increasing accuracy of CR data a number of anomalies have appear with respect to the standard paradigm of propagation of charged particles in the Galaxy. In this thesis, we demonstrate that some of these anomalies disappear by taking into account the systematic uncertainties involving these kind of analyses, specially cross sections uncertainties.

==> Glosary.tex <==
%\chapter*{\vspace{-6cm}\hspace{-4cm}Glossary of keywords}
\chapter*{Glossary of keywords}
\label{ch:Gloss}
\addcontentsline{toc}{chapter}{Glossary of Keywords} 

\large{\textbf{\hspace{0.82cm}Primary cosmic ray:}}	Those cosmic rays whose which are injected by the sources. For example, protons, oxygen, carbon, neon nuclei.
%\vskip 3.5mm

\textbf{Injection spectrum:} Energy spectrum at which a cosmic ray element exits from the acceleration source and is injected to the interstellar medium.
%\vskip 3.5mm

\textbf{Secondary cosmic ray:} Those cosmic rays which principally are formed via spallation reactions. In general, a secondary particle is created from the collision of a primary particle and a pure secondary nuclei is not injected at the sources. Typical examples are B, Be and Li.
%\vskip 3.5mm

\textbf{Spallation reactions:} Hadronic, inelastic reactions between a projectile CR and nuclei from the ISM (as target) which generate and eject at least a product nucleus. Typically spallation interactions are associated to the fragmentation of the target nucleus. 

%\textbf{Inelastic reaction:}

\textbf{Grammage:} Amount of matter traversed by cosmic rays in their propagation path. Its units are [$g/cm^2$].

\textbf{Ghost nuclei:} Those unstable nuclei, generated via spallation reactions, whose lifetime negligible compared to typical propagation times, and their contribution is directly added up to the formation of their daughter nuclei.

\textbf{Direct spallation cross sections:} Spallation cross sections of prompt production of a species of cosmic ray nuclei.

\textbf{Cumulative spallation cross sections:} 
Spallation cross sections which add the contribution from the decay of  ghost nuclei to the prompt production. While a direct reaction is $^{12}C + p \longrightarrow ^{11}C + X$, the cumulative reaction for $^{11}B$ production is $^{12}C + p \longrightarrow ^{11}C + X \hspace{0.5 cm} {\xrightarrow{\makebox[1.5cm]{fast decay}}} \hspace{0.4cm} ^{11}B$.

\textbf{Main spallation channels:} Those spallation reaction channels which are dominant for the production of a particular isotope of a secondary nuclei. As an example, spallation reactions with $^{12}C$ and $^{16}O$ as projectiles account for more than 50\% of the total flux of B, Be and Li.

\textbf{Secondary spallation channels:} Those spallation reaction channels from primary cosmic ray isotopes other than $^{12}C$ and $^{16}O$, which account usually by less than $\sim5\%$ to the total production of a particular secondary particle.

\textbf{Tertiary spallation channels:} Those spallation reaction channels with a secondary cosmic ray isotope as projectile producing another cosmic ray isotope.

\textbf{Local cosmic-ray spectrum:} Spectrum of cosmic rays measured in the Earth's vicinity.



==> approval.tex <==
\chapter*{}
\thispagestyle{empty}
\vspace{-1in}
\begin{center}
{\Large  {\bf Thesis Approval}}
\end{center}
\vspace*{0.1in} \noindent This thesis entitled {\large \bf Thesis title} by {\bf \large
Student Name} is approved for the degree of  {\large \bf Doctor of Philosophy}.\\\\
\hspace*{4 in} Examiners:\\\\
\hspace*{3.5 in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots\\\\
\hspace*{3.5 in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots\\\\
\hspace*{3.5 in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots\\\\
  \hspace*{3.5in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots\\\\
 Supervisor:\hspace*{3.5 in}  Chairperson:\\\\\\
\ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots
\hspace*{1.0 in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
\ldots \ldots \ldots\ldots\\\\\\
%  \hspace*{4 in} Chairman:\\\\
% \hspace*{3.8 in} \ldots\ldots \ldots \ldots \ldots \ldots\ldots
% \ldots \ldots \ldots\ldots

\noindent
Date: \ldots\ldots \ldots \ldots\\\\
Place: \ldots\ldots \ldots \ldots
%\pagebreak \clearpage{\pagestyle{empty}\cleardoublepage}
% \clearpage{\pagestyle{empty}\cleardoublepage}


==> chap_07_List_of_Publications.tex <==
\chapter*{Related publications}
\label{ch:pub}
\addcontentsline{toc}{chapter}{\nameref{ch:pub}}

A paper dedicated to chapter \ref{sec:XSecs} is under preparation. For the paper...
   
\section*{International Journals}
\begin{enumerate}
	
	\item Bhattacharya. A, \textbf{Surendar. M}, 2016,\textquotedblleft Enhanced Target Detection and Improved Scattering Power Decompositions Using the Optimized Coherency Matrix from Full-Polarimetric SAR Data \textquotedblright, \textit{Geoscience and Remote Sensing Letters, IEEE}, (Under revision)
	
	\item \textbf{Surendar. M}, Bhattacharya. A, Singh. G,  Yamaguchi. Y, 2016,\textquotedblleft Estimation of snow surface dielectric constant from polarimetric SAR data \textquotedblright, \textit{Journal of Selected Topics in Applied Earth Observations and Remote Sensing, IEEE}, (Under revision)
	
	\item Pandey. P, \textbf{Surendar. M}, Bhattacharya. A, Ramanathan. A.L, Singh. G, Venkataraman. G, 2015,\textquotedblleft Qualitative and quantitative assessment of TanDEM-X DEM over western Himalayan glaciated terrain \textquotedblright, \textit{Geocarto International}, (In Press)
	
	
\end{enumerate}
\section*{International Conferences}
  \begin{enumerate}
  \item Banerjee, B, De. S, \textbf{Surendar. M}, Bhattacharya, A, 2016 \textquotedblleft An Unsupervised hidden markov random field based segmentation of polarimetric SAR images\textquotedblright, \textit{Geoscience and Remote Sensing Symposium (IGARSS), IEEE International}, (submitted)
  
  \item Deo. R, \textbf{Surendar. M}, Rao. Y.S, Gedam. S.S, 2013 \textquotedblleft Evaluation of interferometric SAR DEMs generated using TanDEM-X data\textquotedblright, \textit{Geoscience and Remote Sensing Symposium (IGARSS), IEEE International}, pp.2079-2082, 21-26 July 2013 \break doi:10.1109/IGARSS.2013.6723221.

\item \textbf{Surendar. M}, Bhattacharya. A, Singh. G, Venkataraman. G, Bharathi, P.A, 2013 \textquotedblleft Snow wetness estimation from polarimetric SAR image\textquotedblright, \textit{Progress In Electromagnetics Research Symposium (PIERS)}, Stockholm, Sweden, Aug. 12-15, 2013, pp.678-682.

\item \textbf{Surendar. M}, Bhattacharya. A, Venkataraman. G, 2013 \textquotedblleft Glacier Velocity Estimation Using Offset Tracking Method\textquotedblright, \textit{TerraSAR-X/TanDEM-X Science Team Meeting}, DLR, 2013, Oberpfaffenhofen, Germany, https://tandemx-science.dlr.de/pdfs.



\end{enumerate}
%\section*{National Conferences}
%  \begin{enumerate}
%  \item \textbf{S. K. Panda}, S. S. Gedam, and G. Rajaram, 2014, \textquotedblleft Investigations of Geomagnetic storm effect on the equatorial ionospheric anomaly over Indian region with GPS, Radio occultation and magnetometer observations\textquotedblright, \textit{Proc. of  National Conference on Application of  Geoinformatics in Rural, Urban \& Climatic Studies (Geomatrix’14)}, Indian Institute of Technology Bombay, CD proceedings.
%  \item \textbf{S. K. Panda} and S. S. Gedam, 2012, \textquotedblleft Investigating ionospheric total electron content over low latitude Indian region by analysis of GPS signals during ascending part of 24th Solar cycle\textquotedblright, \textit{National Symposium on ‘Space Technology for Food \& Environmental Security’ \& Annual Convention of Indian Society of Remote Sensing \& Indian Society of Geomatics}, Delhi, India, Abstract proceedings.
%\end{enumerate}

==> symbols.tex <==
\chapter*{List of Symbols}
\label{ch:sym}
\addcontentsline{toc}{chapter}{\nameref{ch:sym}}
\makeatletter
%\newcommand{\tocfill}{\cleaders\hbox{$\m@th \mkern\@dotsep mu . \mkern\@dotsep mu$}\hfill}
\makeatother
%\newcommand{\abbrlabel}[1]{\makebox[3cm][l]{\textbf{#1}\ \tocfill}}
\newenvironment{symbols}{\begin{list}{}{\renewcommand{\makelabel}{\abbrlabel}
                                              \setlength{\itemsep}{0pt}}}{\end{list}}
\begin{symbols}
\item[$\mu$] 	Magnetic permeability
\item[$\mu_0$]	Magnetic permeability of free space
\item[$\varepsilon$] Relative complex dielectric constant
\item[$\varepsilon^{'}$]  Real part of dielectric constant 
\item[$\varepsilon^{''}$] Imaginary part of dielectric constant 
\item[$\varepsilon_{s}$] Snow surface dielectric constant
\item[$\varepsilon_{v}$] Snowpack volume dielectric constant
\item[$\kappa_e$] Volume extinction coefficient
\item[$\kappa_{a}$] Absorption coefficient
\item[$\kappa_{s}$]	Scattering coefficient
\item[$\delta_{p}$] Penetration depth
\item[$\delta R$]   Slant range resolution of SAR data
\item[$\delta R_g$]  Ground range resolution of SAR data
\item[$\mbox{c}$]	Speed of light
\item[$\lambda$]	Wavelength
\item[$\tau$] Pulse length of SAR signal
\item[$\beta$]  Bandwidth of the SAR signal
\item[$\theta$ ] 	Orientation angle 
\item[$\theta_{i}$] 	Incidence or local incidence angle
\item[$\theta_{r}$]  Local refractive angle 
\item[$\delta A$]	Azimuth resolution of the SAR data
\item[$L$]    SAR antenna length
\item[$\mathbf{E}(\mathbf{r},t)$] Electric field vector
\item[$\mathbf{E_{pq}^s}$]	Scattered field vector
\item[$\rho(\mathbf{r}, t)$] Volume density of free charges
\item[$\mathbf{g}_\mathbf{E}$] Stokes vector
\item[$g_0$] Total power of the wave
\item[$g_1$] Power in the linear horizontal or vertical polarized components
\item[$g_2$] Power in the linearly polarized components at tilt angles $\psi$= 45$^\circ$ or 135$^\circ$
\item[$g_3$] Power in the left-handed and right-handed circular polarized component
\item[$\mathbf{[J]}$]	Jones matrix
\item[$\bm{U_2}$] Unitary matrix ($\mbox{SU}_2$)
\item[$\lambda_1$, $\lambda_2$]	Non-negative real eigenvalues
\item[$A_W$] Wave anisotropy 
\item[$A_{p}$] Particle anisotropy
\item[$H_W$] Entropy
\item[$\mathbf{[S]}$]	$2\times2$ Sinclair matrix
\item[$\bm{k}$] 3-D Pauli target vector
\item[$\{\Psi_P\}$]	Pauli spin matrix set
\item[$\{\Psi_L\}$]	Lexicographic matrix basis set
\item[$\bm{\varOmega}$]	Lexicographic target vector
\item[$\mathbf{[T]}$]	$3\times3$ Coherency matrix
\item[$\mathbf{[C]}$]	$3\times3$ Covariance matrix
\item[$T^{*}$]	Matrix transpose with complex conjugation (superscript)
\item[$\langle ... \rangle$]	Spatial or temporal ensemble average
\item[$\sigma$$^\circ$]	Backscattering coefficient
\item[$\sigma_{hh}^0$]	Backscattering coefficient of $\mbox{HH}$ polarization
\item[$\sigma_{vv}^0$]	Backscattering coefficient of $\mbox{VV}$ polarization
\item[$\sigma_{vvhh}^0$]	Correlation coefficient between $\mbox{VV}$ and $\mbox{HH}$ polarization
\item[$\alpha_1$]	Dominant scattering magnitude
\item[$\mathbf{[T_2]}$]	$2\times2$ coherency matrix
\item[$m_{E}$]	Effective DOP
\item[$m_{E}^{\mbox{\scriptsize opt}}$]	Optimized AGU-Dop
\item[$p_{max}$]	Touzi optimum Dop (maximum)
\item[$p_{min}$]	Touzi optimum Dop (minimum)
\item[$\chi_{t}^{\mbox{\scriptsize opt}}$]	Optimum polarization angles (ellipticity)
\item[$\psi_{t}^{\mbox{\scriptsize opt}}$]	Optimum polarization angles (orientation)
\item[$s$]	RMS surface roughness
\end{symbols}



